Streaming instabilities in accreting protoplanetary disks: A parameter study

The streaming instability (SI) is currently the leading candidate for triggering planetesimal formation in protoplanetary disks. Recently, a novel variation, the `azimuthal-drift' streaming instability (AdSI), was discovered in disks exhibiting laminar gas accretion. Unlike the classical SI, the AdSI does not require pressure gradients and can concentrate dust even at low abundances. We extend previous simulations of the AdSI to explore the impact of dust abundance, accretion flow strength, pressure gradients, and grain size. For a dimensionless accretion flow strength $\alpha_{\mathrm{M}}=0.1$ and particle Stokes number $\operatorname{St}=0.1$, we find the AdSI produces dust filaments for initial dust-to-gas ratios as low as $\epsilon=0.01$. For $\epsilon\gtrsim 1$, maximum dust-to-gas ratios of order 100 are attained, which can be expected to undergo gravitational collapse. Furthermore, even in systems dominated by the classical SI, an accretion flow drives filament formation, without which the disk remains in a state of small-scale turbulence. Our results suggest that an underlying accretion flow facilitates dust concentration and may thus promote planetesimal formation.

==> scratch.tex <==
% In this study, we mainly follow the step in \cite{Hsu22} but broaden the parameter space in the simulation. We find that although the $\delta \rho_{d,max}/\rho_0$ value seems to conserve at $\sim 60$ P for their fiducial case E3eta0am001 (It also can be seen in Fig.\ref{fig:deltarhod} in Appendix.\ref{sec:density_perturbation}), the growth is still ongoing until $T\sim100$ P. We extend the simulation time up to $150$ P to make sure the disk has already reached the steady state.
% As a consequence work of \cite{Hsu22}, we make the overall result more complete. We show that with an appropriate magnetic stress, local dust density can be increased by at most 100 times. For dust-poor disk with initial $\epsilon \geq0.1$, AdSI can enhance the dust density to reach the strong clumping condition. 
% We also verify their result of turbulent coefficients, and find that $\alpha_{g,y}$ is the dominant term with $\sim2$ order of magnitude larger than diffusion of other directions. However, for angular momentum term, $\alpha_{SS}$ is not necessary to be equal to diffusion term.
% \mkl{comparison with bai and stone 2010 on role of radial pressure gradient}
% Previous study with stratified disks showed that strong radial pressure gradient disfavor clumping, because the turbulence is too strong and stir up dust particles \citep{Bai10}. With presence of both radial pressure gradient and magnetic field, the clumping condition is no longer hold at $\rho_{d,max}/\rho_0=100$. We suggest that the AdSI is suppressed by radial pressure gradient in the disk initially with low dust-to-gas ratio. For the disk with high dust-to-gas ratio, AdSI can make some extra increase of dust-to-gas ratio, but not as efficient as classical SI due to the strong turbulence. However, The exception appear at the region close to the pressure bump, showing that AdSI can become efficiently in disk with both high and low dust-to-gas ratio. 
% Consider the accreting disk with vanish radial pressure gradient, our simulations show that with a sufficient magnetic stress (usually in the range $0.1<\alphaM<1$, based on our result), AdSI can increase the local dust-to-gas ratio by the maximum 100 times. If we compare Fig.\ref{fig:overview} and Fig.\ref{fig:am_eps_anal}, we can see some correlation between simulation and analytical result. Although we discuss in the previous section that the exact value of growth rate in linear theory is not the same as the value in simulation, the trend of the magnitude is very similar. Therefore, we can utilize this to make our following discussion. For example, in the theory medium $\epsilon$ and high $\alphaM$ lead to high growth rate, and this can be applied to our simulation. With such initial conditions disk can evolve very rapidly to reach the growth upper bound, whereas with low $\alphaM$ the growth rate is relatively low and AdSI either no present in the disk or require more time to raise the local metallicity.  


%\subsection{Main parameters and fiducial values}
% We describe parameters that characterize the disk in this section. For simplicity, in the following description, we take off subscript $0$ of all notations that we only focus on variables evaluated in equilibrium state. We fix the disk aspect ratio $\hgas=H_g/R$ to $0.05$. 

% By considering the components of radial and azimuthal magnetic field $B_R$ and $B_\phi$ in \cite{Lin22}, we can have the expression of Lorentz force in radial and azimuthal direction 
% \begin{equation}
%     F_R=-\frac{B_\phi^2}{2\mu_0 R \rho_\mathrm{g}},
% \end{equation}
% \begin{equation}
%     F_{\phi}=\frac{B_R B_{\phi}}{2\mu_0 R \rho_\mathrm{g}},
% \end{equation}
% with magnetic permeability $\mu_0$ and $B_R B_{\phi} < 0$. 

% For magnetic field, we write plasma beta as
% \begin{equation}
%     \beta_{\phi}=\frac{\mu_0\rho_\mathrm{g} C_s^2}{B^2}=\frac{C_s^2}{C_{A\phi}^2},
% \end{equation}
% where $C_{A\phi}^2=B^2/\mu_0\rho_\mathrm{g}$ is defined as azimuthal Alfv\'en speeds. We then describe the Ohmic resistivity by using Elsasser numbers 
% \begin{equation}
%     \Lambda_{\phi}=\frac{C_s^2}{\eta_O\beta_{\phi}\Omega}.
% \end{equation}
% In the above equation, $\eta_O$ is constant diffusion coefficient.

% We then can define the dimensionless Maxwell stress as
% \begin{equation}
%     \alphaM=-\frac{2RF_{\phi}}{C_s^2}=\frac{\hgas^2}{2\Lambda_{\phi}\beta_{\phi}^2},
% \end{equation}
% in here we consider only the azimuthal drift triggered by large-scale, horizontal magnetic torques interacting with the gas, but $F_{\phi}$ can still apply in other context. For example, if the radial gas accretion resulted from vertical angular momentum loss equivalent to that induced by a corresponding $F_{\phi}$ \citep{McNally17}, then our results can still work.


%\mkl{runs initialized with eps=100 should easily meet the clumping condition. what does it mean when you label them as clumping? there should probably be another condition for a system to qualify as `clumping', i.e. if filaments form. to be discussed.}

%For runs `Eps100am0.01' and `Eps100am0.001', we do not find appreciable instability and the system remains close to its initial state.\mkl{label these as "stable"} 

% \begin{table}[htbp]
% \caption{Parameter setups in our simulations.}\label{sim_summary}
% \setlength\tabcolsep{10pt}
% \begin{tabularx}{\linewidth}{ l l l c}
% \hline\hline
% Run            & $\epsilon$           & $\alphaM$                   & End state status  \\
% \hline
% Eps0.1am1      &  0.1               &  1                           &  Turbulent                \\
% Eps0.1am0.1    &  0.1               &  0.1                         &  Turbulent                \\
% Eps0.1am0.01   &  0.1               &  0.01                        &  Unsaturated                \\
% Eps0.1am0.001  &  0.1               &  0.001                       &  Unsaturated                \\
% Eps0.01am1     &  0.01              &  1                           &  Unsaturated                \\
% Eps0.01am0.1   &  0.01              &  0.1                         &  Unsaturated                \\
% Eps0.01am0.01  &  0.01              &  0.01                        &  Unsaturated                \\
% Eps0.01am0.001 &  0.01              &  0.001                       &  No SI                \\
% Eps1am1        &  1                 &  1                           &  Clumping                \\
% Eps1am0.1      &  1                 &  0.1                         &  Clumping                \\
% Eps1am0.01     &  1                 &  0.01                        &  Turbulent                \\
% Eps1am0.001    &  1                 &  0.001                       &  Turbulent                \\
% Eps10am1       &  10                &  1                           &  Clumping                \\
% Eps10am0.1     &  10                &  0.1                         &  Clumping                \\
% Eps10am0.01    &  10                &  0.01                        &  Clumping                \\
% Eps10am0.001   &  10                &  0.001                       &  No SI                \\
% Eps100am1      &  100               &  1                           &  Clumping                \\
% Eps100am0.1    &  100               &  0.1                         &  Clumping                \\
% Eps100am0.01   &  100               &  0.01                        &  No SI/Clumping                \\
% Eps100am0.001  &  100               &  0.001                       &  No SI/Clumping                \\
% \hline\hline
% \end{tabularx}
% \label{table:parameters}
% \end{table}



% We can also compare the growth rate of these cases. From the figure we can see that if we have lower initial $\epsilon$, it require more time to reach the stable state. These results are predicted by the analytical methods, where the density growth is proportional to the dust-to-gas ratio, and the growth rate is also positive relative to the dust-to-gas ratio. We will describe more in Sec.\ref{sec:disscussion}.
% The above relation can also be applied in high initial $\epsilon$ case. For $\epsilon =10$ (yellow line), the density growth is an order of magnitude larger than the growth of fiducial case.  



% We do not consider the case with too high or too low $\epsilon$ as we discuss before that the dust density is too high to have significant growth in $\epsilon=100$ case, and the system is not yet converge in $\epsilon=0.01$ case. Fig.\ref{fig:delta_rhod_normalized_alpha0.01} also show that even with low $\alphaM$, the AdSI can still increase the dust density by $\sim30$ times.



% especially in high $\epsilon$ cases ($\epsilon=100$), there are over 30 filaments in this state and $\rho_{d,max} \geq 100\rho_0$, allowing the gravitational collapse. 
% At the steady state ($T=100$P) the high initial dust-to-gas ratio will lead to more dense and low-spacing filaments. This might happen because of the instability speed is very low while $\epsilon$ is large. Therefore the filaments are nearly stay at the origin place and hard to merge with nearby filaments. 
% Moving to $\epsilon=10$ and $1$, these two cases only have 3 and 1 filaments respectively, but each filament has a large width. For the case with $\epsilon=0.1$, which does not meet the clumping condition, it still concentrate the dust to form the filaments, but cannot merge into a big enough structure to reach the clumping condition. 
% For $\epsilon=0.01$, although there are multiple filaments in this case, but we think the large spacing between filaments ($>0.05H_g$) makes them hard to merge with each other within simulation timescale. Hence, the AdSI cannot efficiently increase the dust density.

%Another consideration is that if the dust rings undergo sufficiently high azimuthal wavenumber instabilities ---> if they happen on very small scales then they may not be observable 

% \mkl{as epsilon decreases you get more rings. so maybe rings become more closely spaced with increasing distance from the star, since usually epsilon decreases with R}

%Let us examine the properties of the single dust ring formed in our simulation with $\alphaM=0.1$, $\epsilon=0.1$, and $\widetilde{\eta}=0$ (see Fig. \mkl{???}). \mkl{plot the radial profile of density and alphaR. test dullemond's ring model using alphaR. does alphaR differ inside and outside the rings? what is the expected thickness of the dust layer for the measured alphaZ? commentary on ring width --- is it actually observable?} 

%However, these studies consider dust-trapping pressure bumps, which differ from AdSI dust rings that do not involve pressure variations \mkl{this is true? check if AdSI dust rings are associated with pressure bumps}. 

% According to Fig.\ref{fig:ringwidth}, the location of overdensed regions are quite similar so it shows that arising local dust density can result in local gas accretion. However, since the scale of gas density perturbation is too weak, we cannot conclude that it is efficient for dust to raise the local gas density.


%\mkl{what is the diffusion coefficient inside the dust ring?} \scw{around $3.x*10^{-7}$, in the same order of magnitude}

% For turbulent coefficient, we adopt $\alpha_{g,x}$ in the equation since it is the most relevant term that tend to diffusive the rings radially. 
%With the maximum local $\epsilon\sim10^3$ in our fiducial case (see Fig.\ref{fig:ringwidth}), the analytical result shows that $a_{\mathrm{d}}/a_{\mathrm{g}} \cong 0.6$ under the same given conditions in our simulation, which is quite similar to our previous simulation result. This indicates Eq.\ref{eq:ringwidth} appropriately predict the ring widths according to their current conditions.

% \subsection{Vertical structure of the disk} \label{sec:Vertical_Structure}

% \mkl{***MKL editing bookmark***}

% Our simulations  non-stratified disk. To consider more realistic disk (i.e. stratified disk) by adopting the turbulence strength of our fiducial case $\alpha_{g,z}\sim10^{-6}$, which is much less than $\st$, we can find the vertical particle scale height 
% \begin{equation}
%    \frac{H_{\mathrm{d}}}{H_{\mathrm{g}}}=\sqrt{\frac{\alpha_{\mathrm{g},z}}{\OmK \st}},
% \end{equation}
% using the diffusion model in \cite{Dubrulle95}, which gives $H_{\mathrm{d}}\sim0.003H_{\mathrm{g}}$. To be more general, if we consider the cases listed in Table \ref{table:turbulent} in a stratified disk, the maximum vertical scale height $H_{\mathrm{d}}\sim0.01H_{\mathrm{g}}$. Our selected simulation box size is then sufficient to resolve the whole disk structures.



% \subsection{Efficiency for dust to gas ratio of AdSI} \label{sec:AdSI_efficiency}
% \mkl{moved to section 2 since this is linear theory}

